A Model for Minimizing Active Processor Time

We introduce the following elementary scheduling problem. We are given a collection of n jobs, where each job has an integer length as well as a set Ti of time intervals in which it can be feasibly scheduled. Given a parameter B, the processor can schedule up to B jobs at a timeslot t so long as it is "active" at t. The goal is to schedule all the jobs in the fewest number of active timeslots. The machine consumes a fixed amount of energy per active timeslot, regardless of the number of jobs scheduled in that slot (as long as the number of jobs is non-zero). In other words, subject to all units of each job being scheduled in its feasible region and at each slot at most B jobs being scheduled, we are interested in minimizing the total time during which the machine is active. We present a linear time algorithm for the case where jobs are unit length and each Ti is a single interval. For general Ti, we show that the problem is NP-complete even for B = 3. However when B = 2, we show that it can be efficiently solved. In addition, we consider a version of the problem where jobs have arbitrary lengths and can be preempted at any point in time. For general B, the problem can be solved by linear programming. For B = 2, the problem amounts to finding a triangle-free 2-matching on a special graph. We extend the algorithm of Babenko et. al. to handle our variant, and also to handle non-unit length jobs. This yields an O(sqrt(L)m) time algorithm to solve the preemptive scheduling problem for B = 2, where L is the sum of the job lengths. We also show that for B = 2 and unit length jobs, the optimal non-preemptive schedule has at most 4/3 times the active time of the optimal preemptive schedule; this bound extends to several versions of the problem when jobs have arbitrary length.

==> linear.tex <==
\def\Ip.{I$'$}
% -- ICALP edit 02/18/2012 -- wording of this whole section 
%We conclude this section by showing the algorithm 
%can be implemented in time $O(n+T)$.
%We start by giving the following equivalent version of  Phase I, which we
We define Phase \Ip. %as an equivalent version of Phase I:
to be equivalent to Phase I:
%refer to as Phase \Ip.:
initially each deadline value has no jobs assigned to it.
Process jobs $j$ in order of decreasing release time,
%Jobs with the same release time can be processed in arbitrary order.
assigning $j$ to a new deadline equal to the largest value $D\le d_j$ that
has $<B$ jobs assigned to it.  
We now argue their equivalence.

%To show Phase \Ip. computes the same deadlines as
%Phase I, assume that both algorithms break ties
%in the same way.  
Let $D$ ($D^*$, respectively) be the deadline assigned
to job $j$ in Phase \Ip. (Phase I).
%We prove that each
%iteration of Phase \Ip. computes $D$ as Phase I's deadline $D^*$
%the deadline assigned to job $j$ by Phase I.
%assigned to job $j$.
%Suppose this holds for all iterations preceding
% -- ICALP edit 02.20.2012.06 -- next line
Suppose for jobs $i$, $i < j$, $i$'s Phase I and Phase \Ip.
deadlines are equal.
Then $D^*\le D$ by Phase \Ip.'s choice of $D$.
%Consider  Phase I when it assigns jobs  new
%deadline values equal to $D = D_j$.  It 
Phase I first assigns $D$ 
to the $<B$ jobs currently assigned
$D$ in Phase \Ip., since they have release time $\ge r_j$.
Among all jobs which can still be assigned $D$, 
$j$ has the latest release time.  So $D^*=D$.
% -- ICALP edit 02.19.2012.01 -- this par
We implement Phase \Ip. in $O(n+T)$ time
using a disjoint set merging algorithm \cite{GTSet}.
%on the universe of possible
%deadline values $1..T$. Each set consists of a deadline $D$
%that has been assigned to $<B$ jobs, plus the
%maximal set of consecutive values $D+1,\ldots$
%that have each been assigned to $B$ jobs.
%Then by \cite{GTSet},%it is easy to see
%Phase \Ip. runs in $O(n+T)$ time.
%using the set merging data structure of
%\cite{GTSet}.
%achieves time
%$O(n+T)$ for Phase \Ip..

% -- ICALP edit 02/18/2012 -- many wording changes in this para.
%Phase II constructs an EDF
%schedule on the timeslots that are Phase I deadlines.
%In detail, 
Let $D_1<D_2<\ldots <D_\ell$ be the distinct
deadline values assigned to jobs in Phase I.
Phase II % modifies release times and deadlines 
compresses the active interval
from $[0,T]$ to $[0,\ell]$, as follows: job $j$ with
Phase I deadline $D_k$ gets deadline $k$; its %given
release time
$r_j$
changes to the largest integer $i$ with
$D_i\le r_j$ (let $D_0=0$).
The algorithm returns the EDF schedule
on this modified instance, %. It returns that schedule, with
with slot $i$ changed back to $D_i$.
Phase II assigns new release times
in time $O(n+T)$ and constructs an EDF schedule via
disjoint set merging,
% -- ICALP edit 02.19.2012.01 -- cut out reference to Phase \Ip.
% as in Phase \Ip.,
% -- ICALP edit 02/18/2012b.10 -- removed Fred citation
% \cite{Fred},
achieving time  $O(n+T)$ \cite{GTSet}.

